Posit NPB: Assessing the Precision Improvement in HPC Scientific Applications

Floating-point operations can significantly impact the accuracy and performance of scientific applications on large-scale parallel systems. Recently, an emerging floating-point format called Posit has attracted attention as an alternative to the standard IEEE floating-point formats because it could enable higher precision than IEEE formats using the same number of bits. In this work, we first explored the feasibility of Posit encoding in representative HPC applications by providing a 32-bit Posit NAS Parallel Benchmark (NPB) suite. Then, we evaluate the accuracy improvement in different HPC kernels compared to the IEEE 754 format. Our results indicate that using Posit encoding achieves optimized precision, ranging from 0.6 to 1.4 decimal digit, for all tested kernels and proxy-applications. Also, we quantified the overhead of the current software implementation of Posit encoding as 4x-19x that of IEEE 754 hardware implementation. Our study highlights the potential of hardware implementations of Posit to benefit a broad range of HPC applications.

==> evaluation.tex <==
\section{Experimental Setup}\label{sec:evaluation}
We evaluate the benchmarks in different precision on a workstation with an Intel Core i7-7820X CPU with eight cores and 16 threads. The system has 32GB of RAM with a 480GB SSD. The operating system is Fedora 29 running on Kernel version 4.19.10-300. The compiler used is GCC 8.2.1 and the latest SoftPosit library from main development branch is used\footnote{SoftPosit commit 688cfe5d}. We compute the machine epsilon ($\epsilon$) of different formats using linear search with the "plus one" method for reference. On this workstation, the measured $\epsilon$ values are 1.926E-34, 2.220E-16, 1.192E-07, 7.450E-09 and for \code{quad}, \code{double}, \code{float} and \code{posit32} respectively.

Reproducing floating-point computation results across platform and optimization is a difficult task. When compiling the benchmarks, we have used the flags \code{-ffp-contract=off} for turning off possible Fused Multiply Add (FMA) and \code{-ffloat-store} to avoid storage of floating-point variables in registers thus avoiding the effect of storing intermediate value in extend precision by the processor. We select three problems for evaluation, size S, W and A. The only changes we have made is the number of iterations in order to evaluate their lowest achievable error. We also modified the verification of MG, LU and BT to use $L_2$ error norm instead of Root Mean Square Error. Specifications of the problems can be referred to the original specification~\cite{bailey1991parallel}. 

%We evaluate precision loss and error in different ways depending of the application:

%{\bf CG: Conjugate Gradient.}
%We developed five versions of the CG kernels where computation is performed using \code{quad}, \code{double}, \code{float} and \code{posit32}. We extend the version of \code{posit32} and perform dot product in \code{quire32} to improve accumulation accuracy. We compute the explicit residual norm at the end of each CG iteration with $L_2$ norm $||Error|| = ||x - Az||$ in quad precision. At the end of each Inverse Power Iteration, we compute the error $|\zeta - \zeta_{truth}|$ between the reference answer and $\zeta$ in quad precision. We note that the residual norm being used by the algorithm is still computed in their native precision. We retained the implementation of $A$ matrix generation and the generated values are converted to the respective precision used. We perform 30 Inverse Power iterations, which is equivalent to 750 CG iterations.
%
%{\bf FT: Fast Fourier Transform.}
%In the case of FT, verification is performed in form of a checksum. For this reason, the verification method is not suitable for quantifying error due to change in precision. Instead, we perform verification through an element-by-element comparison of result state arrays. At each step, the $L_2$ norm of the result state array is computed using the results from quad precision as ground truth. We first compute the distance between every element between the truth and the computed solution with $\sqrt{x^2+y^2}$ where $x$ is the real and $y$ the imaginary part of a complex number. Then the $L_2$ norm is computed using those values. Furthermore, since the time stepping process is discrete and does not depend on results from the previous step, we only perform one time step as the process does not quantify propagation of error due to time stepping.
%
%{\bf MG: Multigrid.}
%In the case of MG, since the residual vector is a part of the solver, the vector is computed in native precision while the $L_2$ residual norm is computed in Quad precision. We execute the solver for 100 iterations.
%
%{\bf LU: LU Solver.}
%For LU, verification is performed by computing the $L_2$ error norm of the solution of the PDEs. Exact solutions of the PDEs using the exact method are computed then compared with the approximated solution after every iteration. The exact solution and comparison is computed and performed using Quad precision. However the initial values and boundary values are computed in their native precision. We define the error of the iteration to be the highest error out of the five errors and present the highest $L_2$ norm out of the five PDEs as the error of an iteration.. We execute the solver for 2500 iterations.
%
%{\bf BT: Block Tridiagonal Solver.}
%Similarly to LU, BT verification is performed by computing the $L_2$ error norm of the solution of the PDEs. We compute the exact solution in Quad precision after every iteration and compute the $L_2$ error norm of approximated solutions. The Right Hand Side is still computed in native precision using the exact method. We define the error of the iteration to be the highest error out of the five errors. We execute the solver for 2500 iterations.
